Video Anomaly Detection using GAN

Accounting for the increased concern for public safety, automatic abnormal event detection and recognition in a surveillance scene is crucial. It is a current open study subject because of its intricacy and utility. The identification of aberrant events automatically, it's a difficult undertaking because everyone's idea of abnormality is different. A typical occurrence in one circumstance could be seen as aberrant in another. Automatic anomaly identification becomes particularly challenging in the surveillance footage with a large crowd due to congestion and high occlusion. With the use of machine learning techniques, this thesis study aims to offer the solution for this use case so that human resources won't be required to keep an eye out for any unusual activity in the surveillance system records. We have developed a novel generative adversarial network (GAN) based anomaly detection model. This model is trained such that it learns together about constructing a high dimensional picture space and determining the latent space from the video's context. The generator uses a residual Autoencoder architecture made up of a multi-stage channel attention-based decoder and a two-stream, deep convolutional encoder that can realise both spatial and temporal data. We have also offered a technique for refining the GAN model that reduces training time while also generalising the model by utilising transfer learning between datasets. Using a variety of assessment measures, we compare our model to the current state-of-the-art techniques on four benchmark datasets. The empirical findings indicate that, in comparison to existing techniques, our network performs favourably on all datasets.

==> Algo/FCM.tex <==
 \begin{table}[h!]
 \Large
\centering
\begin{tabular}{l l} 
 \hline
 Notation & Description\\ [0.5ex] 
 \hline
  $x_i$ & $i^{th}$ data point\\
  $N$ & number of data points \\
  $C$ & number of clusters \\
  $p$ & fuzzification parameter \\
  $u_{ij}$ & membership of $i^{th}$ data point to the $j^{th}$ cluster\\
  $T$ & number of iterations for algorithm to converge \\
  $v_j$ & centroid of $j^{th}$ cluster \\ [1ex]
 \hline
\end{tabular}
\caption{ \large Major Math Symbols - FCM Clustering}
\end{table}

\begin{algorithm}[H]
\Large
\caption{ \Large \ \ Fuzzy C-Means Algorithm}\label{alg:FCM}
\begin{algorithmic}[1]
\Require Points: $\{ x_1..., x_N \} $, No. of clusters: $K$, Fuzzification parameter: $p$
\State Initialize Membership values $\mu_{ij}$ randomly
\State $T = 0 $
\Repeat 
\State $T = T +1$
\For{ $j = 1$ to $C$  }
\vspace{0.25cm}
\State $v_j = \frac{\sum\limits_{i=1}^{N} (u_{ij})^p x_i}{\sum\limits_{i=1}^{N} (u_{ij})^p}$
\vspace{0.25cm}
\Comment{Update cluster centroid }
\EndFor 
\For{ $i = 1$ to $N$ }
\For{ $j = 1$ to $C$}
\vspace{0.25cm}
    \State $u_{ij}= \frac{1}{\sum\limits_{k=1}^C \left( \frac{|| x_i - v_j ||}{|| x_i - v_k ||}\right)^{\frac{2}{p-1}}}$
    \Comment{Update Membership values }
\EndFor
\EndFor 
\Until{ convergence}

\end{algorithmic}
\end{algorithm}
The asymptotic time complexity of the algorithm is $\mathcal{O}(NKT)$.

==> Algo/Fuzzy_Inference.tex <==
Algorithm \ref{alg:Fuzzy Inference} given below, defines the steps in the Fuzzy Inference operation in detail.
\begin{table}[H]
\Large
\centering
\begin{tabular}{l l} 
 \hline
 Notation & Description\\ [0.5ex] 
 \hline
  $I$ & Array of pixels\\
  $K$ & Number of fuzzy sets in first layer \\
  $P_k$ & Membership Matrix for $k^{th}$ fuzzy set \\
  $\overline{P_k}$ & Firing Strength for $k^{th}$ fuzzy set \\ 
  $F1, F2, F3, F4$ & Fuzzy Sets \\  [1ex]
 \hline
\end{tabular}
\caption{ \large Major Math Symbols- Fuzzy Inference Operation}
\end{table}

\begin{algorithm}[H]
\Large
\caption{ \large Fuzzy Inference Operation}\label{alg:Fuzzy Inference}
\begin{algorithmic}[1]
\Require Image: $I$, FilterSet1: $F1$, FilterSet2: $F2$, FilterSet3: $F3$, FilterSet4: $F4$
\Ensure 
\State $K = len(F1)$
\For{ $k=1$ to $K$ }
\State $P_k$ = $I \circledast F1_k $   \Comment{Membership Matrix}
\State ${P_k}$ = clip($P_k$)       \Comment{Clipping to [0,1]}
\EndFor 
\For{$k=1$ to $K$ }
\For{$i=1$  to $len({P_k})$ }
    \State $\overline{p_{ik}}= \frac{p_{ik}}{\sum\limits_{j=1}^K {p_{ij}}}$
    \Comment{Firing Strength}
\EndFor
\EndFor 
\State $T_1 = (\overline{P_1} \ \overline{P_2} \ ........\ \overline{P_k})$ 
\State $T_2 = Padding(T_1)$      \Comment{Padding} 
\State $T_2 = T_2 \circledast F2$ 
\State $g = T_2 \circledast F3$
\State $f = I \circledast F4$
\State $y = g \circledast f$   
\State \Return $y$
\end{algorithmic}
\end{algorithm}

==> Algo/Fuzzy_Pooling.tex <==
Algorithm \ref{alg:Fuzzy Pooling} given below, defines the steps in the Fuzzy Pooling operation in detail.
\begin{table}[H]
\Large
\centering
\begin{tabular}{l l} 
 \hline
 Notation & Description\\ [0.5ex] 
 \hline
  $I$ & Array of pixels\\
  $K$ & Number of fuzzy sets in first layer \\
  $P_k$ & Membership Matrix for $k^{th}$ fuzzy set \\
  $\overline{P_k}$ & Firing Strength for $k^{th}$ fuzzy set \\
  $F1, F2, F3$ & Fuzzy Sets \\ [1ex]
 \hline
\end{tabular}
\caption{\large Major Math Symbols- Fuzzy Inference Operation}
\end{table}

\begin{algorithm}[H]
\Large
\caption{\large Fuzzy Pooling Operation}\label{alg:Fuzzy Pooling}
\begin{algorithmic}[1]
\Require Image: $I$, FilterSet1: $F1$, FilterSet2: $F2$, FilterSet3: $F3$
\Ensure 
\State $K = len(F1)$
\For{ $k=1$ to $K$ }
\State $P_k$ = $I \circledast  F1_k $   \Comment{Membership Matrix}
\State ${P_k}$ = clip($P_k$)       \Comment{Clipping to [0,1]}
\EndFor 
\For{$k=1$ to $K$ }
\For{$i=1$  to $len({P_k})$ }
    \State $\overline{p_{ik}}= \frac{p_{ik}}{\sum\limits_{j=1}^K {p_{ij}}}$
    \Comment{Firing Strength}
\EndFor
\EndFor 
\State $T_1 = (\overline{P_1} \ \overline{P_2} \ ........\ \overline{P_k})$ 
\State $T_2 = T_2 \circledast F2$ 
\State $g = T_2$
\State $f = I \circledast F3$
\State $y = g \circledast f$   
\State \Return $y$
\end{algorithmic}
\end{algorithm}

==> Algo/K_means.tex <==
Algorithm \ref{alg:Algorithm 1 K-Means} defines the K-Means algorithm below.
\begin{Large}
\begin{table}[h!]
\large
\centering
\begin{tabular}{l l} 
 \hline
 Notation & Description\\ [0.5ex] 
 \hline
  $x_i$ & $i^{th}$ data point\\
  $N$ & number of data points \\
  $K$ & number of clusters \\
  $\mu _i$ & centroid of $i^{th}$ cluster \\
  $T$ & number of iterations for algorithm to converge \\
  $z_i$ & cluster to which $x_i$ data point is assigned \\ [1ex]
 \hline
\end{tabular}
\caption{\large Major Math Symbols- K-Means Clustering}
\end{table}

\begin{algorithm}[H]
\large
\caption{\large K-Means Algorithm}\label{alg:Algorithm 1 K-Means}
\begin{algorithmic}[1]
\Require Data points: $\{ x_1, x_2 ..., x_N \} $, Number of clusters: $K$
\Ensure Set of $K$ clusters
\State Initialize cluster centroids $\mu_1$,$\mu_2$...$\mu_K$ randomly
\State $ T = 0 $
\Repeat 
\State $  T = T + 1 $
\For{ $i = 1$ to $N$ }
    \State $ z_i = argmin_k ||\mu_k -x_i ||^2 $
     \Comment{Assign data points to clusters}
\EndFor 

\For{ $j = 1$ to $K$  }
\vspace{0.25cm}
 \State $\mu_j = \frac{\sum\limits_{i=1}^N \{ z_i = k \} x_i  }{ \sum\limits_{i=1}^N \{ z_i = k \} } $
 \Comment{Update Cluster Centroids}
\vspace{0.25cm}
\EndFor 
\Until{ convergence}
\end{algorithmic}
% \label{alg:K-Means}
\end{algorithm}
The asymptotic time complexity of the $K$-Means Algorithm is $\mathcal{O}(NKT)$. \\
\end{Large}

==> Algo/dynamic_image.tex <==
\begin{Large}
As discussed in section \ref{VideoSummary}, we use Dynamic image generation to summarize a video using rank pooling techniques as formulated by Bilen et al.~\cite{Bilen2016}. \\ \\
Let us consider a video to have frames, say, $F_1, F_2,...F_C$. The number of frames in the whole video is C. We will consider the feature vector extracted from $F_i$ as $\phi(F_i) \in \mathbb{R}^{d}$. The 3 RGB components of an image are given as input to the operator $\phi(F_i)$. It stacks the pixel values onto a single vector.\\ \\
 Each frame, $F_i$ is given a rank, and a video is represented in terms of the ranks of its frames. Let $\overline{\phi_i} = \frac{1}{i} \sum\limits_{j=1}^{i}\phi(F_j)$. Let each frame $F_i$ be given a score $\psi(i,\lambda) = \langle\ \overline{\phi_i},\lambda \rangle $ where $\lambda \in \mathbb{R}^{d}$ is a vector of parameters. Frames that appear earlier in the video are given lower scores than the frames that appear later in the video, \textit{i.e.}, $\psi(i,\lambda) < \psi(j,\lambda)$ for $i < j$. These function parameters $\lambda^*$ are learned. The scores thus achieved reflect the rank of the frames in the video. Let us use the idea of RankSVM to learn $\lambda^*$. The optimization problem can be formulated as:\\
\begin{equation}
 \lambda^* = \operatorname*{argmin}_\lambda U(\lambda).  
\end{equation} \\
\[ U(\lambda) = \frac{\alpha}{2} ||\lambda||^2 + \frac{2}{C(C-1)} \times \sum_{i > j} max\{1+\psi(j,\lambda)-\psi(i,\lambda), 0 \} \] \\ \\
The second term is a soft counting hinge loss function that counts incorrectly ranked pairs of points. For this, we consider all points whose score values differ by at least one unit, \textit{i.e.}, $\psi(i,\lambda) - \psi(j,\lambda) > 1 $. We call this process of computing $\lambda^*$ rank pooling. \\ \\
Computing a dynamic image involves solving the optimization problem in eq.(1). To solve the optimization problem much faster, consider the first step in gradient-descent optimization. Starting with $\lambda = \vec{0}$, we obtain:
\[ \lambda^* = \sum_{i=1}^{C} w_i \phi(F_i) \]
where the coefficients $w_i$ are given by:
\begin{equation}
\delta_i = 2(C - i +1) - (i+1)(\tau_i - \tau\textsubscript{i-1} )
\end{equation}\\ 
where $ \tau_i = \sum\limits_{j=1}^{i} \frac{1}{j} $ is the $i^{th}$ Harmonic number, and $\tau_0 = 0$. After approximation, the calculation of $\lambda^*$ is equivalent to the weighted summation of the feature vectors $\phi(F_i)$. This is called approximate rank pooling.
\end{Large}
